Accelerating Serverless Computing by Harvesting Idle Resources

Serverless computing automates fine-grained resource scaling and simplifies the development and deployment of online services with stateless functions. However, it is still non-trivial for users to allocate appropriate resources due to various function types, dependencies, and input sizes. Misconfiguration of resource allocations leaves functions either under-provisioned or over-provisioned and leads to continuous low resource utilization. This paper presents Freyr, a new resource manager (RM) for serverless platforms that maximizes resource efficiency by dynamically harvesting idle resources from over-provisioned functions to under-provisioned functions. Freyr monitors each function's resource utilization in real-time, detects over-provisioning and under-provisioning, and learns to harvest idle resources safely and accelerates functions efficiently by applying deep reinforcement learning algorithms along with a safeguard mechanism. We have implemented and deployed a Freyr prototype in a 13-node Apache OpenWhisk cluster. Experimental results show that 38.8% of function invocations have idle resources harvested by Freyr, and 39.2% of invocations are accelerated by the harvested resources. Freyr reduces the 99th-percentile function response latency by 32.1% compared to the baseline RMs.

==> implementation.tex <==
\section{Implementing \sys}

\sys provides a general resource management service for functions in serverless platforms. 
For concreteness, we describe its implementation in the context of Apache OpenWhisk framework \cite{openwhisk}. In this section, we briefly introduce the architecture of OpenWhisk, and describe the workflow of \sys managing resources for functions in OpenWhisk system.

\subsection{Integrating \sys with OpenWhisk}
\label{subsec:openwhisk}

Apache OpenWhisk is an open-source, distributed serverless platform which powers IBM Cloud Functions \cite{ibm-cloud-functions}. Figure~\ref{fig:openwhisk} illustrates the architecture of \sys integrated with OpenWhisk. OpenWhisk exposes an NGINX-based REST interface for users to interact with the platform. Users can create new functions, invoke functions, and query results of invocations via the frontend. The Frontend forwards function invocations to the Controller, which selects an Invoker (typically hosted using VMs) to execute invocations. The Load Balancer inside the Controller implements the scheduling logic by considering Invoker's health, available capacity, and infrastructure state. Once choosing an Invoker, the Controller sends the function invocation request to the selected Invoker via a Kafka-based distributed messaging component. The Invoker receives the request and executes the function using a Docker container. After finishing the function execution, the Invoker submits the result to a CouchDB-based Database and informs the Controller. Then the Controller returns the result of function executions to users synchronously or asynchronously. Here we focus on resource management for containers. 

We modify the following modules of OpenWhisk to implement our resource manager:

\textbf{Frontend:} Initially, OpenWhisk only allows users to define the memory limit of their functions and allocates CPU power proportionally based on memory. To decouple CPU and memory, we add a CPU limit and enable Frontend to take CPU and memory inputs from users. Now users are allowed to specify CPU cores and memory of their functions, and the Frontend forwards both CPU and memory limit to Controller.

\textbf{Controller:} The Load Balancer makes scheduling decisions for the Controller. When selecting an Invoker, the Load Balancer considers available memory of Invokers. We modify Load Balancer also to check available CPU cores of Invokers, \ie, now Load Balancer selects Invokers with enough available CPU cores and memory to execute function invocations.

\textbf{Invoker:} The Invoker uses a semaphore-based mechanism to control access of containers to its available memory. To manage CPU independently, we apply the identical mechanism to control access to available CPU cores.

\textbf{Container:} By default, OpenWhisk uses \texttt{cpu-shares} parameter to regulate CPU power of containers. When plenty of CPU cycles are available, all containers with \texttt{cpu-shares} use as much CPU as they need. While \texttt{cpu-shares} improves CPU utilization of Invokers, it can result in performance variation of function executions. We change the CPU parameter to \texttt{cpus} which restricts how many CPU cores a container can use. This is aligned with the CPU allocation policy of AWS Lambda \cite{awslambdalimits}. For each function invocation, we monitor the CPU cores and memory usage of its container using \texttt{cgroups}. We record the usage peak during function execution and keep it as history for \sys to query.

\subsection{Implementing RL Agent in \sys}
\label{subsec:freyr-workflow}

\sys communicates with OpenWhisk Controller directly via a Key-Value (KV) Store implemented using Redis. When receiving a function invocation, the Load Balancer in the Controller first sends the current state information to the KV Store. The DRL Agent in \sys then fetches the state and sends an action back to Controller. After Controller picks up the action, the Load Balancer adjusts the resource allocation of the function invocation based on the action provided by \sys, and then forwards it to a chosen Invoker for execution. Because \sys is a resource manager inside serverless platforms, we make \sys communicate with the Controller rather than the Frontend. This reduces communication overhead and speeds up the training.

We implement the prototype of \sys agent using two neural networks; each with two fully-connected hidden layers. The first hidden layer has 32 neurons, and the second layer has 16 neurons; each neuron uses \texttt{Tanh} as its activation function. The agent of \sys is implemented in Python using PyTorch \cite{pytorch}. \sys uses multiprocessing to retrieve results of function invocations for computing rewards. The implementation of \sys is lightweight as the policy network consists of 1858 parameters (12 KBs in total) because \sys reuses the score network. Mapping a state to an action takes less than 50 ms. \note{talk more about the bottleneck between Python and Scala, and the actual latency of the RL agent.}

We use the algorithm presented in Section~\ref{subsec:training} to train \sys with 4 epochs per surrogate optimization and a 0.2 clip threshold \cite{ppo2}. We update the policy network parameters using the AdamW optimizer \cite{adamw} with a learning rate of 0.001. 
For simulation, We train \sys over 5000 episodes. For OpenWhisk experiment, we train \sys with 500 episodes. The total time for OpenWhisk training takes about 120 hours. We restart the OpenWhisk platform before each training episode. Figure~\ref{fig:loss} shows the learning curve of \sys training in simulation and OpenWhisk experiment, respectively. The descending loss trendlines in both indicate that \sys gradually learns to make good resource management decisions for functions through training.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.45\linewidth]{figures/sim-loss.pdf}
%     \caption{The cumulative average loss of \sys in simulation through 5000 episodes.}
%     \vspace{-0.2in}
%     \label{fig:loss-sim}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.45\linewidth]{figures/openwhisk-loss.pdf}
%     \caption{The cumulative average loss of \sys in OpenWhisk experiment through 500 episodes.}
%     \vspace{-0.2in}
%     \label{fig:loss-openwhisk}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[t]{0.48\linewidth}
%         \includegraphics[width=\textwidth]{figures/sim-loss.pdf}
%         \caption{\sys training in simulation through 5000 episodes.}
%     \end{subfigure}
%     % \hfill
%     \begin{subfigure}[t]{0.48\linewidth}
%         \includegraphics[width=\textwidth]{figures/openwhisk-loss.pdf}
%         \caption{\sys training in OpenWhisk through 500 episodes.}
%     \end{subfigure}
%     \vspace{-0.1in}
%     \caption{Learning curves of \sys training in simulation and OpenWhisk evaluation.}
%     \vspace{-0.2in}
%     \label{fig:loss}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{figures/loss.eps}
%     \vspace{-0.25in}
%     \caption{The cumulative average loss of \sys in the 5000-episode simulation and 500-episode OpenWhisk training, respectively.}
%     \label{fig:loss}
% \end{figure}
